Restructuring, Pruning, and Adjustment of Deep Models for Parallel Distributed Inference

Using multiple nodes and parallel computing algorithms has become a principal tool to improve training and execution times of deep neural networks as well as effective collective intelligence in sensor networks. In this paper, we consider the parallel implementation of an already-trained deep model on multiple processing nodes (a.k.a. workers) where the deep model is divided into several parallel sub-models, each of which is executed by a worker. Since latency due to synchronization and data transfer among workers negatively impacts the performance of the parallel implementation, it is desirable to have minimum interdependency among parallel sub-models. To achieve this goal, we propose to rearrange the neurons in the neural network and partition them (without changing the general topology of the neural network), such that the interdependency among sub-models is minimized under the computations and communications constraints of the workers. We propose RePurpose, a layer-wise model restructuring and pruning technique that guarantees the performance of the overall parallelized model. To efficiently apply RePurpose, we propose an approach based on $\ell_0$ optimization and the Munkres assignment algorithm. We show that, compared to the existing methods, RePurpose significantly improves the efficiency of the distributed inference via parallel implementation, both in terms of communication and computational complexity.

==> Contributions.tex <==
We depart from the traditional methods by focusing on the restructuring and manipulation of the model for more efficient parallel implementation. 
%
Without changing the general topology of the neural network, we propose to rearrange the neurons and partition the deep model into sub-models with minimum co-dependency subject to the computation and communication constraints on the workers.
%
%\begin{figure}
%	\centering
%	\begin{overpic}[width=\linewidth]{Figures/ModelRestructuring_Example}
%		\put (5,-5) {\scalebox{.9}{(a) Original model}} 
%		\put (55,-5) {\scalebox{.9}{(b) Restructured model}} 
%	\end{overpic}
%	~
%	\caption{Restructuring a neural network to reduce communication between processing units}
%	\label{fig:RestructuringModel}
%	\vspace{-5mm}
%\end{figure}
%%
%As an example, consider the simple neural network in Fig.~\ref{fig:RestructuringModel}(a). Simple partitioning the model into two sub-models (as depicted by a dashed line in the figure) imposes lots of communication between the two sub-models. However, by rearranging the neurons properly, the co-dependency (and hence required communications) between two workers (as indicated by the red edges in Fig.~\ref{fig:RestructuringModel}(b)) is reduced substantially.

==> RePurposeS.tex <==
In this section, we introduce and analyze two variants of the RePurpose algorithm which acts in the \emph{parameter space} or \emph{signal space}. 
In the first approach, to have the modified neural network perform similar to the original one, we require that the modified parameters $\whvect{W}$ be close to the permuted parameters of the original model (i.e., $\vect{W\Pi}^\Tr$). In the second method, inspired by \cite{Aghasi2017Net,Aghasi2020Fast}, we analyze the signals passing through the neural network to ensure that the outcomes of the modified neural network is close to the original one.

\subsection{Signal Space RePurpose}
Here, instead of using the closeness of the modified parameters to the original ones, we consider the behavior of the neural network for given input data. We examine the closeness of the signals passing through the layers of the neural network as the measure of similarity between the modified model and the original one. By ensuring that the signals are close, we can guarantee the performance of the modified restructured model (similar to~\cite{Aghasi2017Net,Aghasi2020Fast}).

For an input batch of size $K$, let $\vect{X}$ be the input signals to the $l$-th layer. Assume that $\vect{Y}$ and $\whvect{Y}$ are the corresponding computed signals by the $l$-layer in the original and modified neural network. The objective of RePurpose in Signal-space ({\RPS}) is 
\begin{equation}
\min_{\whvect{W},\whvect{b},\vect{\Pi}} \|\vect{M}\odot\whvect{W}\|_0\quad\quad \subjto~\|\whvect{Y}-\vect{\Pi Y}\|_F^2\leq \epsilon, 
\label{eqn:RePurposeS-OPT}
\end{equation}
where $\epsilon$ is a parameter controlling the closeness of the signal. Similar to~\cite{Aghasi2017Net}, we can show that the above procedure guarantees the performance of the modified neural network.
\begin{theorem}
	Let parameters of an $L$-layer neural network be bounded as $\|\vect{W}^{(l)}\|_F \leq \tau$, $l=1,\ldots,L$. Further, assume that the activation functions are 1-Lipschitz continuous, i.e., $|\sigma(\nu)-\sigma(\omega)|\leq |\nu-\omega|$. Then solving \eqref{eqn:RePurposeS-OPT} for all layers results in a new neural network whose final error is at most $\epsilon \sum_{l=0}^{L-1} \tau^l$.
\end{theorem}
Similar to {\RPP}, we consider the Lagrangian form of \eqref{eqn:RePurposeS-OPT} and add an optional extra term for the total sparsity of the parameters. Hence, the objective would be 
\begin{equation}
	\min_{\vect{\Pi}, \whvect{W}, \whvect{b}} \|\whvect{W}^\Tr\vect{X}+\whvect{b}-\vect{\Pi Y}\|_F^2 + \eta_1 \|\whvect{W}\|_0 + \eta_2 \|\vect{M}\odot\whvect{W}\|_0.
	\label{eqn:Original_RePurposeS}
\end{equation} 

To solve \eqref{eqn:Original_RePurposeS}, first we note the for a given $\whvect{W}$ and $\vect{\Pi}$, the optimum $\whvect{b}$ can be computed as
\begin{equation}
	\whvect{b}=\frac{1}{L} (\vect{\Pi Y}-\whvect{W}^\Tr\vect{X})\vect{1}_{L\times 1} 
	=\vect{\Pi \overline{y}}-\whvect{W}^\Tr\vect{\overline{x}},
\end{equation}
where $\vect{\overline{x}}$ and $\vect{\overline{y}}$ are the averages of the signals at each neuron. As a result, by subtracting the signals' averages (i.e., $\vect{X}\leftarrow\vect{X}-\vect{\overline{x}\,1}^\Tr$, and $\vect{Y}\leftarrow\vect{Y}-\vect{\overline{y}\,1}^\Tr$), the optimization problem to find the permutation and adjusted parameters can be rewritten as 
\begin{equation}
	\min_{\vect{\Pi}, \whvect{W}} \|\whvect{W}^\Tr\vect{X}-\vect{\Pi Y}\|_F^2 + \eta_1 \|\whvect{W}\|_0 + \eta_2 \|\vect{M}\odot\whvect{W}\|_0.
	\label{eqn:Simplified_RePurpose-S}
\end{equation} 
%
Unfortunately, \eqref{eqn:Simplified_RePurpose-S} is NP-hard as it is combinatorial and non-convex due to the $\ell_0$ quasi-norm and the permutation matrix $\vect{\Pi}$. Therefore, we use convex-relaxation technique to efficiently solve it;
\begin{itemize}[leftmargin=12pt,itemsep=1pt,partopsep=1pt,parsep=1pt,topsep=0.5pt]
	\item We relax the $\ell_0$ quasi-norm to $\ell_1$ norm. 
	\item A permutation matrix is a doubly-stochastic matrix with the largest Frobenius norm. Therefore, we relax the permutation matrix $\vect{\Pi}$ to matrix $\vect{Q}$ where $0\leq \vect{Q}\leq 1$, $\vect{Q1}=\vect{1}$ and $\vect{Q}^\Tr\vect{1}=\vect{1}$. Further, we add a penalty term $\|\vect{Q}\|_F$ to encourage $\vect{Q}$ becomes more similar to a permutation matrix.
\end{itemize}
Hence, the relaxed convex optimization problem would be
\begin{equation}
	\min_{\vect{Q}\in\set{Q}, \whvect{W}} \|\whvect{W}^\Tr\vect{X}-\vect{Q Y}\|_F^2 + \|\vect{P}\odot\whvect{W}\|_1 {\color{gray}- \lambda\|\vect{Q}\|_F^2},
	\label{eqn:Convex_RePurpose-S}
\end{equation} 
where $\vect{P}=\eta_1+\eta_2\vect{M}$, $\set{Q}$ is the set of all doubly-stochastic matrices and the (optional) last term, $- \lambda\|\vect{Q}\|_F^2$, is added to make the solution of $\vect{Q}$ more similar to a permutation matrix.
However, note that $\lambda$ cannot be arbitrarily large as it makes the optimization problem non-convex. Indeed, one can easily verify that to ensure the convexity of \eqref{eqn:Convex_RePurpose-S}, 
\begin{equation}
	0\leq \lambda \leq \sigma_{\min}(\vect{YY}^\Tr),
\end{equation}
where $\sigma_{\min}(\vect{A})$ is the minimum eigenvalue of the positive semi-definite matrix $\vect{A}$.

\begin{wrapfigure}[27]{r}{0.44\textwidth}
	\vspace{-5mm}	
	\begin{algorithm}[H]
		\SetAlgoLined
		\caption{\small Signal-Space RePurpose}
		\label{alg:RePurposeS}
		\DontPrintSemicolon
		
		\SetKwFunction{FMain}{\Function{RePurposeS}}
		\Fn{\FMain{$\vect{X}$, $\vect{Y}$, $\vect{M}$, $\lambda$, $\rho$}}
		{
			- $\vect{A}\leftarrow (\vect{XX}^\Tr+\rho\vect{I})^{-1}$\;
			- $\vect{B}\leftarrow (\vect{YY}^\Tr-\lambda\vect{I})^{-1}$\;
			- $\vect{C}\leftarrow \vect{XY}^\Tr$\;
			- $\vect{U}_1\leftarrow 0$,~~~$\vect{U}_2 \leftarrow 0$, ~~$\vect{V} \leftarrow 0$,~~~$\vect{T} \leftarrow 0$\;\vspace{1mm}
			\While{Not converged}
			{
				- $\whvect{W} \leftarrow \vect{A}(\vect{CQ}^\Tr+\rho(\vect{V}-\vect{U}_1))$\;
				- $\vect{V} \leftarrow \mathcal{S}_{\vect{P}/\rho} (\whvect{W}+\vect{U}_1)$\;
				- $\vect{Q} \leftarrow \vect{B}(\whvect{W}^\Tr\vect{C}+\rho(\vect{T}-\vect{U}_2))$\;
				- $\vect{T} \leftarrow \mathcal{P}_{\set{Q}} (\vect{Q}+\vect{U}_2)$\;
				- $\vect{U}_1 \leftarrow \vect{U}_1+\whvect{W}-\vect{V}$\;
				- $\vect{U}_2 \leftarrow \vect{U}_2+\vect{Q}-\vect{T}$\;
			}
			\textbf{Return} $\vect{Q}$, $\whvect{W}$\;
		}
	\end{algorithm}
%-----------------------------
	\vspace{1mm}
	\centering
	\includegraphics[width=\linewidth]{Figures/ModelRestructuring_ExampleVariations.pdf}
	\caption{Different permutations of neurons can lead to equivalent distributed structures.}
	\label{fig:EquivalentPermutations}
\end{wrapfigure}
We use Alternating Direction Method of Multipliers (ADMM)~\cite{Boyd2011Distributed} to solve \eqref{eqn:Convex_RePurpose-S}.
Algorithm~\ref{alg:RePurposeS} summarizes the proposed ADMM-based solution for {\RPS}, where $\rho>0$ is the augmented Lagrangian parameter in ADMM, $\mathcal{S}(\cdot)$ is the soft-thresholding operator 
\begin{equation*}
	\mathcal{S}_{\vect{P}/\rho}(\vect{Z}) = \sign(\vect{Z}) \odot \max(|\vect{Z}|-\vect{P}/\rho, \vect{0}),
\end{equation*} 
and $\mathcal{P}_{\mathcal{Q}}(\vect{Z})$ projects the matrix $\vect{Z}$ onto the convex set of doubly-stochastic matrices.

%The optimization problem \eqref{eqn:Convex_RePurpose-S} can be efficiently solved via the following iterative approach:
%\begin{enumerate}[leftmargin=12pt,itemsep=1pt,partopsep=1pt,parsep=1pt,topsep=1pt]%noitemsep,partopsep=1pt,parsep=1pt,topsep=0pt]
%	\item Fixing $\whvect{W}$ and setting $\vect{A}:=\whvect{W}^\Tr\vect{X}$, the solution to $\vect{Q}$ can be efficiently found via solving the following \emph{Linearly Constrained Quadratic Problem}
%	\begin{equation}
%%	\begin{aligned}[l]
%		\min_{\vect{Q}} ~\|\vect{Q Y}-\vect{A}\|_F^2- \lambda\|\vect{Q}\|_F^2, \quad \quad \subjto ~~0\leq \vect{Q}\leq 1,~\vect{Q1}=\vect{1}, ~\vect{Q}^\Tr\vect{1}=\vect{1} 
%%	\end{aligned}
%	\end{equation}
%	\item For a fixed $\vect{Q}$, the optimization problem to find $\whvect{W}$ can be written as
%	\begin{equation}
%		\min_{\whvect{W}} \|\whvect{W}^\Tr\vect{X}-\vect{Q Y}\|_F^2 + \|\vect{P}\odot\whvect{W}\|_1,
%	\end{equation}
%	where $\vect{P}=\eta_1 + \eta_2\vect{M}$. The solution to this problem can be computed via  LASSO~\cite{Tibshirani1996Regression} and its variants.
%\end{enumerate}
%It is worth mentioning that since the problem \eqref{eqn:Convex_RePurpose-S} is convex, the above iterations will converge to the global minimum.
Note that the solution $\vect{Q}$ of \eqref{eqn:Convex_RePurpose-S} is not necessarily a valid permutation matrix. 
Hence, the next step in {\RPS} would be finding the best permutation $\vect{\Pi}$ to approximate $\vect{Q}$. It can be shown that there is an inherent ambiguity in the permutation matrix $\vect{\Pi}$. Permuting the neurons inside a sub-model results in an equivalent form of the distributed model (Fig.~\ref{fig:EquivalentPermutations}). Hence, if there are $n_k$ neurons in the $k$-th sub-model, there are $n_1!\times\ldots\times n_P!$ different optimum permutation matrices that would result in topologically-equivalent sub-models, and any convex combination of these permutations can be a potential solution to the convex-relaxation problem \eqref{eqn:Convex_RePurpose-S}. Indeed, it can be verified that for $\lambda=0$, if there is a unique optimum neuron assignment, the optimum $\vect{Q}$ would be given as $Q_{ij}=1/n_k$ if both neurons $i$ and $j$ are assigned to the $k$-th worker and $Q_{ij}=0$, otherwise. {\RPS} exploits this observation to find the best neuron assignments to the workers.
Therefore, since the neuron assignments to the workers are not affected, this ambiguity does not harm the RePurpose algorithm. 
Finally, the weights $\whvect{W}$ are readjusted accordingly by solving the following (weighted-) LASSO optimization problem~\cite{Tibshirani1996Regression}
\begin{equation}
	\min_{\whvect{W}} \|\whvect{W}^\Tr\vect{X}-\vect{\Pi Y}\|_F^2 + \|\vect{P}\odot\whvect{W}\|_1.
\end{equation}
Next results states how many data samples (input batch size $K$) are necessary to find the optimum solution $\whvect{W}$.
\begin{proposition}
	Consider an input data batch of size $K$. Assume that the input signals to the layer, $\vect{X}\in\SetR^{M\times K}$, are i.i.d. sub-Gaussian. If there exists a weight matrix $\whvect{W}\in\SetR^{M\times N}$ with at most $s$ cross-edges between workers, with $K=\BigO(s\log(M/s))$ data samples it can be found.
\end{proposition}

